A Novel Confidence Induced Class Activation Mapping for MRI Brain Tumor Segmentation

Magnetic resonance imaging (MRI) is a commonly used technique for brain tumor segmentation, which is critical for evaluating patients and planning treatment. To make the labeling process less laborious and dependent on expertise, weakly-supervised semantic segmentation (WSSS) methods using class activation mapping (CAM) have been proposed. However, current CAM-based WSSS methods generate the object localization map using internal neural network information, such as gradient or trainable parameters, which can lead to suboptimal solutions. To address these issues, we propose the confidence-induced CAM (Cfd-CAM), which calculates the weight of each feature map by using the confidence of the target class. Our experiments on two brain tumor datasets show that Cfd-CAM outperforms existing state-of-the-art methods under the same level of supervision. Overall, our proposed Cfd-CAM approach improves the accuracy of brain tumor segmentation and may provide valuable insights for developing better WSSS methods for other medical imaging tasks.

==> Section/Related_Works.tex <==


In the past few years, several works have discovered the advantage of obtaining segmentation masks in a weakly-supervised manner. In other words, they aim to capture the pixel-level object segmentation mask with image-level labels only. Most of the existing works are initially based on Class Activation Mapping (CAM), which is a technique for identifying activation regions of a trained network. Broadly speaking, recent CAM methods could be categorized into two categories: 1) post-generated CAM and 2) in-training CAM.


\textbf{Post-generated CAM.} These CAM methods \cite{zhou2016learning,selvaraju2017grad,omeiza2019smooth,wang2020score,ramaswamy2020ablation} train the neural network and generate the activation map separately. They utilize the feature maps from the last convolution layer and generate activation maps for the target object through weighted sum, where the weight is defined differently. Zhou et al. \cite{zhou2016learning} introduced the very first CAM method, which directly defines the trainable weights of the fully-connected layer as the weight of feature maps. As an extension, Grad-CAM \cite{selvaraju2017grad} was proposed to calculate the gradients between the target class confidence and the feature map and use them as the weights. 
% Different from the \cite{zhou2016learning}, Grad-CAM makes the CAM technique available to almost all kinds of convolution neural architectures. 
However, several works \cite{omeiza2019smooth,wang2020score} pointed out that Grad-CAM leads to generating low-quality and noisy activation maps. 
In addition, Wang et al. \cite{wang2020score} proposed the ScoreCAM, and pointed out that the activation maps with higher weights would show a lower contribution to the prediction score.
Following-up works have discovered the potential of directly generating segmentation results from these activation maps in medical images. For example, Nguyen et al. \cite{nguyen2019novel} and Kang et al. \cite{kang2021towards} applied thresholding and refinement on the activation map to obtain the final segmentation result. 

\textbf{In-training CAM.} Different from Post-generated CAM, in-training CAM methods \cite{wang2020self,lee2021lfi,zhang2018adversarial,tang2021m} train the neural network and generate the activation map simultaneously. They reveal that object localization maps can be conveniently obtained by directly selecting from the feature maps of the last convolutional layer through the network itself, which no longer requires an extra step to generate an activation map. 
Zhang et al. \cite{zhang2018adversarial} first proposed to produce class-specific activation maps during the forward pass. In addition, they used two adversary classifiers to find the entire object region, rather than barely focusing on a small region. 
% Wang et al. \cite{wang2020self} introduced a self-supervised equivariant attention mechanism to keep the consistency of the network for generating activation maps. Similarly, based on Wang et al., Tang et al.\cite{tang2021m} included the concept of multiple-instance learning and neighborhood affinity module to improve the training efficiency and the accuracy of the activation map.
Lee et al. \cite{lee2021lfi} borrow the concept of ScoreCAM to propose the LFI-CAM, which claimed to learn the score more efficiently. Moreover, they leveraged the attention mechanism to improve the classification performance and generated a more consistent attention map during the forward propagation.



As mentioned in Section \ref{sec:intro}, most of the CAM methods generate the object localization map from the internal information of the neural network, which can lead to inferior solutions.
In addition, most of them still suffer from false activation on negative cases. Thus, the proposed Cfd-CAM redesigns the weight of feature maps by the confidence of masking it to the input test image (Details are introduced in Section \ref{sec:methodology}).


